Multi-Source Multi-Path HTTP (mHTTP): A Proposal

Today, most devices have multiple network interfaces. Coupled with wide-spread replication of popular content at multiple locations, this provides substantial path diversity in the Internet. We propose Multi-source Multipath HTTP, mHTTP, which takes advantage of all existing types of path diversity in the Internet. mHTTP needs only client-side but not server-side or network modifications as it is a receiver-oriented mechanism. Moreover, the modifications are restricted to the socket interface. Thus, no changes are needed to the applications or to the kernel. As mHTTP relies on HTTP range requests, it is specific to HTTP which accounts for more than 60% of the Internet traffic. We implement mHTTP and study its performance by conducting measurements over a testbed and in the wild. Our results show that mHTTP indeed takes advantage of all types of path diversity in the Internet, and that it is a viable alternative to Multipath TCP for HTTP traffic. mHTTP decreases download times for large objects up to 50%, whereas it does no harm to small object downloads.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We introduced mHTTP, a protocol on top of HTTP, which takes advantage of all
types of diversity in the Internet. We provided a prototype implementation of
our proposal and its evaluation. Our measurements over a testbed and in the
wild showed that mHTTP efficiently utilizes the existing path diversity in the
Internet, reduce content delivery latency, and is a viable alternative
to MPTCP. We plan to extend our study to other use cases such as a streaming
content delivery (e.g., YouTube and/or Netflix) from multiple data sources.
Specifically, we are interested in studying if using mHTTP can reduce the
start-up latency of streaming contents~\cite{RAO11-NCO}.


